Non-local parameterization of atmospheric subgrid processes with neural networks

Subgrid processes in global climate models are represented by parameterizations which are a major source of uncertainties in simulations of climate. In recent years, it has been suggested that machine-learning (ML) parameterizations based on high-resolution model output data could be superior to traditional parameterizations. Currently, both traditional and ML parameterizations of subgrid processes in the atmosphere are based on a single-column approach, which only use information from single atmospheric columns. However, single-column parameterizations might not be ideal since certain atmospheric phenomena, such as organized convective systems, can cross multiple grid boxes and involve slantwise circulations that are not purely vertical. Here we train neural networks (NNs) using non-local inputs spanning over 3$\times$3 columns of inputs. We find that including the non-local inputs improves the offline prediction of a range of subgrid processes. The improvement is especially notable for subgrid momentum transport and for atmospheric conditions associated with mid-latitude fronts and convective instability. Using an interpretability method, we find that the NN improvements partly rely on using the horizontal wind divergence, and we further show that including the divergence or vertical velocity as a separate input substantially improves offline performance. However, non-local winds continue to be useful inputs for parameterizating subgrid momentum transport even when the vertical velocity is included as an input. Overall, our results imply that the use of non-local variables and the vertical velocity as inputs could improve the performance of ML parameterizations, and the use of these inputs should be tested in online simulations in future work.

==> trackchanges-0.7.0/README <==

TrackChanges
Multiple editors in LaTeX.
========================================================================

INTRODUCTION:

  The TrackChanges package consists of two parts:
  1.  A LaTex style file: 
        trackchanges.sty
  2.  A GUI, written in python:
         trackchanges.py

  The style file may be used without the GUI.  The GUI is to be used to
  facilitate accepting, rejecting, or modifying the edits made using the
  commands defined in the style file.

  This packages also includes a command line utility: acceptchanges.py.
  This utility will only work in posix environments.

  Help files are available as part of this package:
    ./documentation/web/help.html

  Documentation is also  available at the TrackChanges website.

  To get the latest version of this sofware go to:
    http://trackchanges.sourceforge.net

========================================================================

LaTeX STYLEFILE:

  INSTALLATION:
    Copy the style file to the directory with your LaTeX document.
    The style file can be found at: ./LatexPackage/trackchanges.sty

  USAGE:
    Add the following line to you latex document:
      \usepackage{trackchanges}

    Add the names of the editors in the preamble [OPTIONAL]:
      \addeditor{editor}

    Now you have access to all of the TrackChanges commands:
      \add[editor]{added text}
      \remove[editor]{removed text}
      \change[editor]{removed text}{added text}
      \note[editor]{note text}
      \annote[editor]{text to annotate}{note text}

    See the documentation or website for display options.

========================================================================

TRACKCHANGES GUI

  This is a Beta version of the TrackChanges GUI. 
  That means: Beware! Bugs may lurk ahead.

  If you choose to use this software plese be careful to back up your 
  TeX files.  This software has not been thoroughly tested and may
  corrupt your TeX files.  (The style file is fine and can't mess any
  thing up but the GUI for accepting/rejecting/modifying might.)

  ----------------------------------------------------------------------
  
  WARNING:  
    This program has not be generalized to handle international
    characters.  Such characters may cause unexpected behavior.
  
  NOTE:
    So far the GUI has only been tested on Windows XP and Os X.
    While it should work on linux, it might not.
  
  WARNING (AGAIN):
    This is beta software. It has not been tested much.
    Things may be broken.
  
  
  
  ----------------------------------------------------------------------
  INSTALLATION:
    Once you have all the dependencies installed, 
    just run ./PythonPackage/trackchanges.py
    
      $> cd PythonPackage
      $> python trackchanges.py
  
  
  ----------------------------------------------------------------------
  DEPENDANCIES:
    To get the trackchanges GUI to run you will need several things:
     
    1. Python 2.6 or later
    2. PyQt 4.4.4 or later
  
  ----------------------------------------------------------------------
  WHERE TO GET DEPENDANCIES:
    Python 2.6  -- http://www.python.org/
    PyQt 4      -- http://www.riverbankcomputing.co.uk/
  
  


========================================================================

This file is part of TrackChanges
Copyright 2009 Novimir Antoniuk Pablant
               Felix Salfner

TrackChanges is free software: you can redistribute it and/or modify
it under the terms of the GNU General Public License as published by
the Free Software Foundation, either version 2 of the License, or
(at your option) any later version.

TrackChanges is distributed in the hope that it will be useful,
but WITHOUT ANY WARRANTY; without even the implied warranty of
MERCHANTABILITY or FITNESS FOR A PARTICULAR PURPOSE.  See the
GNU General Public License for more details.

You should have received a copy of the GNU General Public License
along with TrackChanges.  If not, see <http://www.gnu.org/licenses/>.

------------------------------------------------------------------------
